Guiding LLMs The Right Way: Fast, Non-Invasive Constrained Generation

To ensure that text generated by large language models (LLMs) is in an expected format, constrained decoding proposes to enforce strict formal language constraints during generation. However, as we show in this work, not only do such methods incur performance overhead during generation, but many of them also significantly impair task accuracy, if they do not correctly align the underlying LLM sub-word vocabularies with external constraints. To address this, we present a novel decoding algorithm, DOMINO, that can enforce constraints in a fully subword-aligned fashion, while leveraging pre-computation and speculative decoding to achieve virtually no overhead and in some cases even almost 2$\times$ speedup over unconstrained decoding -- thereby outperforming existing approaches by a wide margin.

==> related.tex <==
\section{Related Work} \label{sec:related}

Next, we discuss related approaches in greater detail, again focusing on regex, CFG and now also JSON Schema.

\paragraph{Regex Decoding}
As noted before, many frameworks support regex guided decoding.
\lmql \citep{Beurer-Kellner023} and \synchromesh \citep{PoesiaP00SMG22} implement regular expressions with 
Notable here is \citet{WillardL23}, who use a deterministic finite automaton (DFA) obtained via the standard NFA construction pre-computed offline.

\paragraph{Summary and Commparision}
\cref{tab:constrained_decoding_methods} summarizes the methods discussed in \cref{sec:token_misalignment} and here.



\todo{further approaches like lew}





























